Ramified inverse and planar monoids

Ramified monoids are a class of monoids introduced by the authors. The main motivation for considering these monoids comes from knot theory, see [3, 4, 5]. Thus, in [2] we have studied the ramified monoids of the symmeytric group and of the Brauer monoid, among others. This paper study the ramified of the inverse symmetric monoid, which plays a notable role in knot theory as well, see [10]. Here is also introduced the notion of planar ramified monoid. In particular, we give presentations for some planar ramified monoids arising from noncrossing set partitions.

==> Ramified Inverse and Planar Monoids/pics.tex <==
%\usepackage[
%	externalize=1,
%	font=0.5
%]{../../../Projects/LaTeX/strands20221227}

\newcommand{\aspdf}{1}

\newcommand{\figureone}{
	\ifnum\aspdf=1
		\includegraphics{pics/082.pdf}\qquad
		\includegraphics{pics/000.pdf}
	\else
		\begin{tikzpicture}[scale=1.2]
			\arcpartition[tkzpic=0]{{1,4},{2,3,5}}
		\end{tikzpicture}
		\begin{tikzpicture}[scale=1.2]
			\permutation[tkzpic=0]{1,2,3,4,5}
			\tie[snake=true,snakelen=4,style=solid]{{1,0.3},{4,0.3}}
			\tie[snake=true,snakelen=4,style=solid]{{2,0.7},{3,0.7},{5,0.7}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figuretwo}{
	\ifnum\aspdf=1
		\includegraphics{pics/001.pdf}\kern+1.4em
		\includegraphics{pics/002.pdf}\kern+1.4em
		\includegraphics{pics/003.pdf}\kern+1.4em
		\includegraphics{pics/004.pdf}\kern+1.4em
		\includegraphics{pics/005.pdf}\kern+1.4em
		\includegraphics{pics/006.pdf}
	\else
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{1,2}
		\end{tikzpicture}\kern+1.4em
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{1,3}
		\end{tikzpicture}\kern+1.4em
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{1,4}
		\end{tikzpicture}\kern+1.4em
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{2,3}
		\end{tikzpicture}\kern+1.4em
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{2,4}
		\end{tikzpicture}\kern+1.4em
		\begin{tikzpicture}
			\permutation[tkzpic=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{3,4}
		\end{tikzpicture}
	\fi
}

\newcommand{\figurethr}{
	\ifnum\aspdf=1\[
		\vcdraw{	\includegraphics{pics/007.pdf}}\kern+0.7em=
		\vcdraw{	\includegraphics{pics/008.pdf}}\kern+0.7em\cdot\kern+0.4em
		\vcdraw{\includegraphics{pics/009.pdf}}\kern+0.7em\cdot\kern+0.4em
		\vcdraw{\includegraphics{pics/010.pdf}}\]
	\else\[
		\vcdraw{	\begin{tikzpicture}[scale=1.2]
			\permutation[tkzpic=0]{1,2,3,4,5}
			\tie[snake=true,snakelen=4,style=solid]{{1,0.3},{4,0.3}}
			\tie[snake=true,snakelen=4,style=solid]{{2,0.7},{3,0.7},{5,0.7}}
		\end{tikzpicture}}\kern+0.7em=
		\vcdraw{\begin{tikzpicture}[scale=1.2]
			\permutation[tkzpic=0]{1,2,3,4,5}
			\tie[snake=true,snakelen=4,style=solid]{1,4}
		\end{tikzpicture}}\kern+0.7em\cdot\kern+0.4em
		\vcdraw{\begin{tikzpicture}[scale=1.2]
			\permutation[tkzpic=0]{1,2,3,4,5}
			\tie[snake=true,snakelen=4,style=solid]{2,3}
		\end{tikzpicture}}\kern+0.7em\cdot\kern+0.4em
		\vcdraw{\begin{tikzpicture}[scale=1.2]
			\permutation[tkzpic=0]{1,2,3,4,5}
			\tie[snake=true,snakelen=4,style=solid]{3,5}
		\end{tikzpicture}}\]
	\fi
}

\newcommand{\figurefou}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/011.pdf}}\kern+0.7em*\kern+0.4em
		\vcdraw{\includegraphics{pics/012.pdf}}\kern+0.7em=\kern+0.4em
		\vcdraw{\includegraphics{pics/013.pdf}}\kern+0.7em=\kern+0.4em
		\vcdraw{\includegraphics{pics/014.pdf}}\]
	\else\[
		\vcdraw{\vpartition[height=1.4,type=2]{{-1,1,5},{2,4,-5},{-3,-4}}}*\kern+0.7em*\kern+0.4em
		\vcdraw{\vpartition[height=1.4,type=2]{{1,4},{3,2,-2,-1},{5,-5,-3}}}\kern+0.7em=\kern+0.4em
		\vcdraw{\begin{tikzpicture}
			\vpartition[floor=1,height=0.7,tkzpic=0,type=1]{{-1,1,5},{2,4,-5},{-3,-4}}
			\vpartition[height=0.7,tkzpic=0,type=-1]{{1,4},{3,2,-2,-1},{5,-5,-3}}
		\end{tikzpicture}}\kern+0.7em=\kern+0.4em
		\vcdraw{\vpartition[height=1.4,type=2]{{5,1,-1,-2},{2,4,-5,-3}}}\]
	\fi
}

\newcommand{\figurefiv}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/015.pdf}}\kern+0.6em=\kern+0.4em
		\vcdraw{\includegraphics{pics/016.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/017.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/018.pdf}}\]
	\else\[
		\vcdraw{\permutation{3,1,4,2}}=\kern-1em
		\vcdraw{\permutation{2,1,3,4}}*\kern-1em
		\vcdraw{\permutation{1,2,4,3}}*\kern-1em
		\vcdraw{\permutation{1,3,2,4}}\]
	\fi
}

\newcommand{\figuresix}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/019.pdf}}\kern+0.6em=\kern+0.4em
		\vcdraw{\includegraphics{pics/020.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/021.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/022.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/023.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=2]{{1,-3},{2,-1},{3,-4}}}=\kern-1.2em
		\vcdraw{\permutation{2,1,3,4}}*\kern-1em
		\vcdraw{\permutation{1,2,4,3}}*\kern-0.3em
		\vcdraw{\vpartition[type=2]{{1,-1},{2,-2},{4,-4}}}\,*\kern-1.1em
		\vcdraw{\permutation{1,3,2,4}}\]
	\fi
}

\newcommand{\figuresev}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/024.pdf}}\kern+0.6em=\kern+0.4em
		\vcdraw{\includegraphics{pics/025.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/026.pdf}}\kern+0.6em*\kern+0.4em
		\vcdraw{\includegraphics{pics/027.pdf}}\kern+0.6em=\kern+0.4em
		\vcdraw{\includegraphics{pics/034.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=2]{{1,-3},{3,-4}}}=\kern-0.5em
		\vcdraw{\vpartition[nstr=4,type=2]{{1,-1},{3,-3},{4,-4}}}\,*\kern-0.5em
		\vcdraw{\vpartition[nstr=4,type=2]{{1,-1},{2,-2},{3,-3}}}\,*\kern-0.5em
		\vcdraw{\vpartition[type=2]{{1,-3},{2,-1},{3,-4},{4,-2}}}=\kern+0.5em
		\vcdraw{\begin{tikzpicture}
			\vpartition[floor=1,height=0.5,nstr=4,tkzpic=0,type=1]{{1,-1},{3,-3}}
			\vpartition[floor=0,height=0.5,type=-1,tkzpic=0]{{1,-3},{2,-1},{3,-4},{4,-2}}
		\end{tikzpicture}}\]
	\fi
}

\newcommand{\figureeig}{
	\ifnum\aspdf=1
		\[\begin{array}{c}
			\includegraphics{pics/098.pdf}\qquad
			\includegraphics{pics/099.pdf}\qquad
			\includegraphics{pics/100.pdf}\qquad
			\includegraphics{pics/101.pdf}\qquad
			\includegraphics{pics/102.pdf}
			\\[0.5cm]
			\includegraphics{pics/028.pdf}\qquad
			\includegraphics{pics/029.pdf}\qquad
			\includegraphics{pics/030.pdf}\qquad
			\includegraphics{pics/031.pdf}
		\end{array}\]
	\else
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{1,1.75},{2,1.75}}
			\tie[snake=true,style=solid]{{2,1.5},{2,1}}
		\end{tikzpicture}
	\qquad
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{2,0.25},{4,0.25}}
			\tie[snake=true,style=solid]{{2,1.5},{2,1}}
		\end{tikzpicture}
	\qquad
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{3,1.75},{4,1.75}}
			\tie[snake=true,style=solid]{{3,1.5},{3,1}}
			\tie[snake=true,style=solid]{{4,1.5},{4,1}}
		\end{tikzpicture}
	\qquad
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{1,0.25},{3,0.25}}
			\tie[snake=true,style=solid]{{3,1.5},{3,1}}
			\tie[snake=true,style=solid]{{4,1.5},{4,1}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figurenin}{
	\ifnum\aspdf=1
		\includegraphics{pics/032.pdf}\qquad
		\includegraphics{pics/033.pdf}
	\else
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{1,1.75},{2,1.75}}
			\tie[snake=true,style=solid]{{2,0.25},{4,0.25}}
		\end{tikzpicture}
	\qquad
		\begin{tikzpicture}
			\permutation[floor=3,height=0.5,tkzpic=0,type=1]{1,2,3,4}
			\vpartition[bulla=0,bullb=0,floor=2,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1}}
			\permutation[floor=1,height=0.5,tkzpic=0,type=0]{2,4,1,3}
			\permutation[bulla=0,height=0.5,tkzpic=0,type=-1]{1,2,3,4}
			\tie[snake=true,style=solid]{{3,1.75},{4,1.75}}
			\tie[snake=true,style=solid]{{3,1.5},{3,1}}
			\tie[snake=true,style=solid]{{1,0.25},{3,0.25}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figureten}{
	\ifnum\aspdf=1\[
		I\,\,=\vcdraw{\includegraphics{pics/035.pdf}}\,\,,\qquad
		J\,\,=\vcdraw{\includegraphics{pics/036.pdf}}\,\,,\qquad
		(I,J)\,\,=\vcdraw{\includegraphics{pics/152.pdf}}
	\]\else\[
		I\,\,=\vcdraw{\vpartition[nstr=5,type=2]{{1,-1},{4,-3}}}\qquad
		J\,\,=\vcdraw{\vpartition[nstr=5,type=2]{{-1,1,2,-5},{-2,3,-4},{-3,4,5}}}\qquad
		(I,J)\,\,=\vcdraw{\begin{tikzpicture}
			\vpartition[nstr=5,type=2,tkzpic=0]{{1,-1},{4,-3}}
			\tie[snake=true,style=solid]{{1,1},{2,1},{5,0}}
			\tie[snake=true,style=solid]{{2,0},{3,1}}
			\tie[snake=true,style=solid,bend=25]{{2,0},{4,0}}
			\tie[snake=true,style=solid]{{4,1},{5,1}}
		\end{tikzpicture}}
	\]\fi
}

\newcommand{\figureele}{
	\ifnum\aspdf=1\[
		\begin{array}{c}
			g^*=\!\vcdraw{\includegraphics{pics/037.pdf}}\,\,,\qquad
			g^*_p=\!\vcdraw{\includegraphics{pics/038.pdf}}
			\\[1cm]
			e=\!\vcdraw{\includegraphics{pics/039.pdf}}\,\,,\qquad
			e'=\!\vcdraw{\includegraphics{pics/040.pdf}}\,\,,\qquad
			r=\!\vcdraw{\includegraphics{pics/041-1.pdf}}	
		\end{array}
	\]\else\[
		\begin{array}{c}
			g^*=\!\vcdraw{\begin{tikzpicture}
				\vpartition[nstr=5,tkzpic=0,type=2]{{1,-1},{4,-3},{3,-2}}
			\end{tikzpicture}}\qquad
			g^*_p=\!\vcdraw{\begin{tikzpicture}
				\vpartition[nstr=5,tkzpic=0,type=2]{{1,-1},{4,-3},{3,-2},{2,-4},{5,-5}}
			\end{tikzpicture}}
			\\[1cm]
			e=\!\vcdraw{\begin{tikzpicture}
				\permutation[tkzpic=0]{1,2,3,4,5}
				\tie[snake=true,snakelen=4,style=solid]{1,2}
				\tie[snake=true,snakelen=4,style=solid]{4,5}
			\end{tikzpicture}}\qquad
			e'=\!\vcdraw{\begin{tikzpicture}
				\permutation[tkzpic=0]{1,2,3,4,5}
				\tie[snake=true,snakelen=4,style=solid]{{1,0.75},{5,0.75}}
				\tie[snake=true,snakelen=4,style=solid]{{2,0.25},{4,0.25}}
			\end{tikzpicture}}\qquad
			r=\!\vcdraw{\begin{tikzpicture}
				\strands[nstr=5,tkzpic=0,type=2,tiesnake=true,tiesnakelen=4,tiestyle=solid]{r1-q2-r4}
			\end{tikzpicture}}
			r'=\!\vcdraw{\begin{tikzpicture}
				\strands[nstr=5,tkzpic=0,type=2,tiesnake=true,tiesnakelen=4,tiestyle=solid]{r1-r2-r4}
				\tie[snake=true,snakelen=4,style=solid]{{3,0},{3,1}}
			\end{tikzpicture}}
		\end{array}
	\]\fi
}

\newcommand{\figuretwe}{
	\ifnum\aspdf=1\[
		\!g\,=\vcdraw{\includegraphics{pics/042.pdf}}
	\]\else\[
		g\,=\,\vcdraw{\begin{tikzpicture}
			\permutation[bullb=0,floor=1,height=0.7,tkzpic=0,type=1]{1,2,3,4,5}
			\tie[floor=1,height=0.7,snake=true,snakelen=4,style=solid]{1,2}
			\tie[floor=1,height=0.7,snake=true,snakelen=4,style=solid]{4,5}
			\strands[floor=0.1,height=0.6,nstr=5,rookextend=0,tkzpic=0,type=0,
				tiesnake=true,tiesnakelen=4,tiestyle=solid]{r1-r2-r4}
			\vpartition[bulla=0,bullb=0,floor=-0.9,height=0.7,nstr=5,tkzpic=0,type=0]
				{{1,-1},{4,-3},{3,-2},{2,-4},{5,-5}}
			\tie[floor=0.1,height=0.6,snake=true,snakelen=4,style=solid]{{3,0.065},{3,1.065}}
			\permutation[floor=-1.9,height=0.7,tkzpic=0,type=-1]{1,2,3,4,5}
			\tie[floor=-1.9,height=0.7,snake=true,snakelen=4,style=solid]{{1,0.7},{5,0.7}}
			\tie[floor=-1.9,height=0.7,snake=true,snakelen=4,style=solid]{{2,0.3},{4,0.3}}
		\end{tikzpicture}}
	\]\fi
}

\newcommand{\figureonethr}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/044.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}
		\kern-0.5em\cdots\kern-1em
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-3},{3,-2},{4,-4}}}
		\kern-0.3em\cdots\kern-1em		
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}\]
	\fi
}

\newcommand{\figureonefou}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/047.pdf}}\cdots\!\!	
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}
		\kern-0.3em\cdots\kern-0.8em
		\vcdraw{\vpartition[type=0]{{1,-1},{3,-3}}}
		\kern-0.3em\cdots\kern-1em		
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}\]
	\fi
}

\newcommand{\figureonefiv}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/084.pdf}
		\includegraphics{pics/083.pdf}
		\includegraphics{pics/049.pdf}
	\]\else\[
		\begin{tikzpicture}
			\arcpartition[tkzpic=0]{{1,8},{2,4,10},{5,6,9}}
			\node at(6,0.3){$\to$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={1,2,3,4,5},
				customlabelsbelow={10,9,8,7,6},
				tkzpic=0,
				type=6
			]{{-1,2,4},{5,-5,-2},{1,-3}}
			\node at(3,0.3){$\leftrightarrow$};
		\end{tikzpicture}
		\vpartition[type=2]{{-1,2,4},{5,-5,-2},{1,-3}}
	\]\fi
}

\newcommand{\figureonesix}{
	\ifnum\aspdf=1\[\left(\,\,
		\vcdraw{\includegraphics{pics/050.pdf}}\,\,\,,\,
		\vcdraw{\includegraphics{pics/046.pdf}}\,\,\,\right)\,\,=\,\,
		\vcdraw{\includegraphics{pics/048.pdf}}\]
	\else\[\left(\!\!\!
		\vcdraw{\vpartition[type=2]{{-1,1,3},{2,-3,-4}}},\!\!\!
		\vcdraw{\vpartition[type=2]{{-4,-3,-1,1,2,3},{4,-2}}}\right)=
		\vcdraw{\begin{tikzpicture}
			\vpartition[tkzpic=0,type=2]{{-1,1,3},{2,-3,-4}}
			\tie[height=0.7,snake=true,snakelen=4,style=solid]{{1,0.85},{2.4,0.85}}
			\tie[height=0.7,snake=true,snakelen=4,style=solid]{{2,0},{4,1.43}}
		\end{tikzpicture}}\]
	\fi
}

\newcommand{\figureonesev}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/045.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=0]{{1,-1}}}
		\kern-0.5em\cdots\kern-1em
		\vcdraw{\begin{tikzpicture}
			\permutation[tkzpic=0,type=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid]{{2,0.5},{3,0.5}}
		\end{tikzpicture}}
		\kern-0.3em\cdots\kern-1em		
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}\]
	\fi
}

\newcommand{\figureoneeig}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/052.pdf}}\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/053.pdf}}\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/085.pdf}}\,\,\,\,*\,\,\,
		\vcdraw{\includegraphics{pics/054.pdf}}
		%\vcdraw{\includegraphics{pics/054.pdf}}\,\,\,\,*\,\,\,
		%\vcdraw{\includegraphics{pics/051.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\permutation[height=1.5,tkzpic=0]{4,1,3,2}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{1.87,0.87},{3.4,0.7}}
			\tie[bend=-30,height=1.5,snake=true,snakelen=4,style=solid]{{2.2,0.6},{3,0.15}}
		\end{tikzpicture}
		\qquad		
		\begin{tikzpicture}
			\permutation[floor=1,bullb=0,height=0.75,tkzpic=0,type=1]{1,2,3,4}
			\permutation[height=0.75,tkzpic=0,type=-1]{4,1,3,2}
			\tie[floor=0.75,snake=true,snakelen=4,style=solid]{{1,0.5},{3,0.5}}
			\tie[floor=0.75,snake=true,snakelen=4,style=solid]{{2,0.25},{4,0.25}}
		\end{tikzpicture}
		\qquad		
		\begin{tikzpicture}
			\permutation[floor=2,bullb=0,height=0.5,tkzpic=0,type=1]{2,1,4,3}
			\permutation[floor=1,bullb=0,height=0.5,tkzpic=0,type=0]{1,3,2,4}
			\permutation[height=0.5,tkzpic=0,type=-1]{1,2,4,3}
		\end{tikzpicture}
		\qquad		
		\begin{tikzpicture}
			\permutation[height=1.5,tkzpic=0,type=2]{1,2,3,4}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{1,2}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{3,4}
		\end{tikzpicture}
		\begin{tikzpicture}
			\permutation[height=1.5,tkzpic=0,type=2]{1,2,3,4}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{1,0.7},{3,0.7}}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{2,0.3},{4,0.3}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figureonenin}{
	\ifnum\aspdf=1\[
		\left(\,\,
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/047.pdf}}\cdots\!\!	
		\vcdraw{\includegraphics{pics/043.pdf}}\,\,\,,\,\,
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/055.pdf}}\cdots\!\!	
		\vcdraw{\includegraphics{pics/043.pdf}}
		\,\,\,\right)\,\,=\,\,
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/056-1.pdf}}\cdots\!\!	
		\vcdraw{\includegraphics{pics/043.pdf}}
		\]
		
	\else\[
		%\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}
		%\vcdraw{\strands[nstr=3,tiesnake=true,tiesnakelen=4,tiestyle=solid,type=0]{q1}}
		\vcdraw{\begin{tikzpicture}
			\vpartition[tkzpic=0,type=0]{{1,-1},{3,-3}}
			\tie[snake=true,snakelen=4,style=solid]{{2,0},{2,1}}
		\end{tikzpicture}}
		%\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}
		\]
	\fi
}

\newcommand{\figuretwenty}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/057.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\strands[nstr=4,type=0]{t2}\]
	\fi
}

\newcommand{\figuretwoone}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/058.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\begin{tikzpicture}
			\strands[nstr=4,type=0,tkzpic=0]{t2}
			\tie[snake=true,snakelen=4,style=solid]{{2.5,0.3},{2.5,0.7}}
		\end{tikzpicture}\]
	\fi
}

\newcommand{\figuretwotwo}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/059.pdf}}
		\quad\to\quad
		\vcdraw{\includegraphics{pics/060.pdf}}
		\quad\to\quad
		\vcdraw{\includegraphics{pics/061.pdf}}
	\]
	\else
		\[\begin{tikzpicture}
			\draw[line width=0.7](0.6,0)to[bend left=15](2.4,0.75)to[bend right=15](4.2,1.5);
			\vpartition[height=1.5,tkzpic=0,type=2,font=0.5]{{1,-1},{2,5},{3,4},{6,7},{-3,-6},{-4,-5},{-7,-8}}
		\end{tikzpicture}
		\qquad
		\begin{tikzpicture}
			\path[draw=black,fill=gray!30,line width=0.7](0,0)--(0.6,0)to[bend left=15](2.4,0.75)to[bend right=15](4.2,1.5)--(3.6,1.5)to[bend left=45](3,1.5)--(2.4,1.5)to[bend left=45](0.6,1.5)--(0,1.5)--cycle;
			\path[draw=black,fill=gray!30,line width=0.7](1.2,1.5)to[bend right=45](1.8,1.5)--cycle;
			\path[draw=black,fill=gray!30,line width=0.7](3.6,0)to[bend left=45](4.2,0)--cycle;
			\path[draw=black,fill=gray!30,line width=0.7](1.2,0)to[bend left=45](3,0)--(2.4,0)to[bend right=45](1.8,0)--cycle;
			\vpartition[height=1.5,nstr=8,tkzpic=0,type=2,font=0.5]{{1,-1}}
		\end{tikzpicture}
		\qquad
		\begin{tikzpicture}
			\vpartition[height=1.5,tkzpic=0,type=2,font=0.5]{{-1,1,3,4}}
			\draw[line width=0.7,dashed](0.6,0)to[bend left=25](1.2,0);
			\draw[line width=0.7](0.6,0)to[bend left=40](0.9,0.25)to[bend left=40](1.2,0);
			\draw[line width=0.7,dashed](0,0)to[bend left=20](0.9,0.75)to[bend right=20](1.8,1.5);
		\end{tikzpicture}\]
	\fi
}

\newcommand{\figuretwothr}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/062.pdf}}\cdots\!\!	
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=0]{{1,-1}}}
		\kern-0.3em\cdots\kern-0.8em
		\vcdraw{
			\begin{tikzpicture}
				\vpartition[type=0,tkzpic=0]{{1,-1},{-2,2},{3,-3},{4,-4}}
				\filldraw(0.6,0.5)circle(0.04);
				\filldraw(1.2,0.5)circle(0.04);
				\draw[line width=0.7](0.6,0.5)--(1.2,0.5);
			\end{tikzpicture}
		}
		\kern-0.3em\cdots\kern-1em		
		\vcdraw{\vpartition[type=0]{{1,-1}}}\]
	\fi
}

\newcommand{\figuretwofou}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/063.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\vcdraw{\vpartition[type=0]{{1,-1}}}
		\kern-0.5em\cdots\kern-1em
		\vcdraw{\begin{tikzpicture}
			\permutation[tkzpic=0,type=0]{1,2,3,4}
			\tie[snake=true,snakelen=4,style=solid,color=blue]{{2,0.5},{3,0.5}}
		\end{tikzpicture}}
		\kern-0.3em\cdots\kern-1em		
		\vcdraw{\vpartition[type=0]{{1,-1},{2,-2}}}\]
	\fi
}

\newcommand{\figuretwofiv}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/064-1.pdf}}\quad\to\quad
		\vcdraw{\includegraphics{pics/066-1.pdf}}\quad\to\quad
		\vcdraw{\includegraphics{pics/067-1.pdf}}
		\]
	\else\[
		\begin{tikzpicture}
			\strands[tkzpic=0,height=0.3,font=0.5,type=1,nstr=8,bullb=0,floor=3.2]{i1}
			\strands[tkzpic=0,height=0.8,font=0.5,type=-1,bulla=0]{t3*t2-t4-t6*t3-t5-t7*t4}
		\end{tikzpicture}
		\begin{tikzpicture}
    			\node at(0,0){\includegraphics{pics/065.pdf}};
    			\node[scale=0.55]at(-1.76,1.963){$1$};
    			\node[scale=0.55]at(-0.56,1.963){$2$};
    			\node[scale=0.55]at(0.64,1.963){$3$};
    			\node[scale=0.55]at(1.84,1.963){$4$};
    			\node[scale=0.55]at(-1.76,-1.935){$1$};
    			\node[scale=0.55]at(-0.56,-1.935){$2$};
    			\node[scale=0.55]at(0.64,-1.935){$3$};
    			\node[scale=0.55]at(1.84,-1.935){$4$};
%
    			\draw[line width=0.7](-1.76,-1.75)--(-1.76,1.75);
			\filldraw(-1.76,-1.75)circle(0.04);
			\filldraw(-1.76,1.75)circle(0.04);
%
			\draw[line width=0.7](-0.56,1.75)--(-0.56,1.30);
			\draw[line width=0.7](-0.56,0.8)--(-0.56,-0.3);
			\draw[line width=0.7](-0.56,-0.8)--(-0.56,-1.75);
			\filldraw(-0.56,1.75)circle(0.04);
			\filldraw(-0.56,1.30)circle(0.04);
			\filldraw(-0.56,0.8)circle(0.04);
			\filldraw(-0.56,-0.3)circle(0.04);
			\filldraw(-0.56,-0.8)circle(0.04);
			\filldraw(-0.56,-1.75)circle(0.04);
%
			\draw[line width=0.7](0.64,1.75)--(0.64,-0.3);
			\draw[line width=0.7](0.64,-0.8)--(0.64,-1.75);
			\filldraw(0.64,1.75)circle(0.04);
			\filldraw(0.64,-0.3)circle(0.04);
			\filldraw(0.64,-0.8)circle(0.04);
			\filldraw(0.64,-1.75)circle(0.04);
%
			\draw[line width=0.7](1.84,1.75)--(1.84,-0.3);
			\draw[line width=0.7](1.84,-0.8)--(1.84,-1.75);
			\filldraw(1.84,1.75)circle(0.04);
			\filldraw(1.84,-0.3)circle(0.04);
			\filldraw(1.84,-0.8)circle(0.04);
			\filldraw(1.84,-1.75)circle(0.04);
%
			\tie[
				%snake=true,
				%snakelen=4,
				style=solid,
				color=black
			]{{-1.92,0.25},{4.06,0.25}}
			\tie[
				%snake=true,
				%snakelen=4,
				style=solid,
				color=black
			]{{0.075,-1.345},{2.075,-1.345}}
			\filldraw[black](-0.56,0.25)circle(0.04);
			\filldraw[black](0.64,0.25)circle(0.04);
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,height=3.5,nstr=4,type=2,tkzpic=0]{{1,-1}}
			\draw[line width=0.7](0.6,3.5)--(0.6,3.05);
			\draw[line width=0.7](0.6,2.55)--(0.6,1.45);
			\draw[line width=0.7](0.6,0.95)--(0.6,0);
			\filldraw(0.6,3.05)circle(0.04);
			\filldraw(0.6,2.55)circle(0.04);
			\filldraw[black](0.6,1.98)circle(0.04);
			\filldraw(0.6,1.45)circle(0.04);
			\filldraw(0.6,0.95)circle(0.04);
%
			\draw[line width=0.7](1.2,3.5)--(1.2,1.45);
			\draw[line width=0.7](1.2,0.95)--(1.2,0);
			\filldraw[black](1.2,1.98)circle(0.04);
			\filldraw(1.2,1.45)circle(0.04);
			\filldraw(1.2,0.95)circle(0.04);
%
			\draw[line width=0.7](1.8,3.5)--(1.8,1.45);
			\draw[line width=0.7](1.8,0.95)--(1.8,0);
			\filldraw(1.8,1.45)circle(0.04);
			\filldraw(1.8,0.95)circle(0.04);
%
			\tie[
				%snake=true,
				%snakelen=4,
				style=solid,
				color=black
			]{{1,1.98},{4,1.98}}
			\tie[
				%snake=true,
				%snakelen=4,
				style=solid,
				color=black
			]{{2,0.38},{3,0.38}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figuretwosix}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/068.pdf}
	\]\else\[
		\begin{tikzpicture}
			\filldraw(-2.4,1)circle(0.04);
			\filldraw(-1.6,1)circle(0.04);
			\filldraw(-1.0,1)circle(0.04);
			\filldraw(-0.4,1)circle(0.04);
			\filldraw(+0.4,1)circle(0.04);
			\filldraw(+1.0,1)circle(0.04);
			\filldraw(+1.6,1)circle(0.04);
			\filldraw(+2.4,1)circle(0.04);
%
			\filldraw(-2.4,0)circle(0.04);
			\filldraw(-1.6,0)circle(0.04);
			\filldraw(-1.0,0)circle(0.04);
			\filldraw(-0.4,0)circle(0.04);
			\filldraw(+0.4,0)circle(0.04);
			\filldraw(+1.0,0)circle(0.04);
			\filldraw(+1.6,0)circle(0.04);
			\filldraw(+2.4,0)circle(0.04);
%
			\draw[line width=0.7](-2.4,1)--(-2.4,0);
			\draw[line width=0.7](-1.6,1)--(-1.6,0);
			\draw[line width=0.7](-1.0,1)--(+1.0,0);
			\draw[line width=0.7](-0.4,1)--(-0.4,0);
			\draw[line width=0.7](+0.4,1)--(+0.4,0);
			\draw[line width=0.7](+1.0,1)--(-1.0,0);
			\draw[line width=0.7](+1.6,1)--(+1.6,0);
			\draw[line width=0.7](+2.4,1)--(+2.4,0);
%
			\node at(-1.95,0.4){$\cdots$};
			\node at(+2.05,0.4){$\cdots$};
			%\node at(+0.05,0.8){$\cdots$};
			\node at(+0.05,0.2){$\cdots$};
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figuretwosev}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/069.pdf}
	\]\else\[
		\begin{tikzpicture}
			\filldraw(-2.4,1)circle(0.04);
			\filldraw(-1.6,1)circle(0.04);
			\filldraw(-1.0,1)circle(0.04);
			\filldraw(-0.4,1)circle(0.04);
			\filldraw(+0.4,1)circle(0.04);
			\filldraw(+1.0,1)circle(0.04);
			\filldraw(+1.6,1)circle(0.04);
			\filldraw(+2.4,1)circle(0.04);
%
			\filldraw(-2.4,0)circle(0.04);
			\filldraw(-1.6,0)circle(0.04);
			\filldraw(-1.0,0)circle(0.04);
			\filldraw(-0.4,0)circle(0.04);
			\filldraw(+0.4,0)circle(0.04);
			\filldraw(+1.0,0)circle(0.04);
			\filldraw(+1.6,0)circle(0.04);
			\filldraw(+2.4,0)circle(0.04);
%
			\draw[line width=0.7](-2.4,1)--(-2.4,0);
			\draw[line width=0.7](-1.6,1)--(-1.6,0);
			\draw[line width=0.7](-0.4,1)--(-0.4,0);
			\draw[line width=0.7](+0.4,1)--(+0.4,0);
			\draw[line width=0.7](+1.6,1)--(+1.6,0);
			\draw[line width=0.7](+2.4,1)--(+2.4,0);
%
			\node at(-1.95,0.4){$\cdots$};
			\node at(+2.05,0.4){$\cdots$};
			%\node at(+0.05,0.8){$\cdots$};
			\node at(+0.05,0.2){$\cdots$};
%
			\tie[
				snake=true,
				snakelen=4,
				style=solid,
				color=red
			]{{-0.66,1},{+2.67,0}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid,
				color=red
			]{{-0.66,0},{+2.67,1}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figuretwoeig}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/070.pdf}}\,\cdots
		\vcdraw{\includegraphics{pics/148.pdf}}
		\kern+1.5em\leftrightarrow\kern+1em
		\vcdraw{\includegraphics{pics/070.pdf}}\,\cdots
		\vcdraw{\includegraphics{pics/071.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=0]{{1},{-1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=0]{{1},{-1},{2},{-2},{3},{-3}}
			\tie[color=blue,style=solid]{{3,0},{3,0}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figuretwonin}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/072.pdf}\,\,
		\includegraphics{pics/073a.pdf}
		\includegraphics{pics/073b.pdf}
	\]\else\[
		\begin{tikzpicture}
			\arcpartition[tkzpic=0]{{1,3,5},{2,7,8},{4,6,9}}
			\filldraw[blue](2.4,0)circle(0.04);
			\node at(5.5,0.3){$\to$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={1,2,3,4,5},
				customlabelsbelow={9,8,7,6,5},
				tkzpic=0,
				type=6
			]{{1,3,5},{2,-2,-3},{4,-4,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\node at(3,0.3){$\to$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				tkzpic=0,
				type=2
			]{{1,3,5},{2,-2,-3},{4,-4,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethirty}{
	\ifnum\aspdf=1\[
		I\,\,=\vcdraw{\includegraphics{pics/074.pdf}}\,\,,\qquad
		J\,\,=\vcdraw{\includegraphics{pics/075.pdf}}\,\,,\qquad
		(I,J)\,\,=\vcdraw{\includegraphics{pics/153.pdf}}
	\]\else\[
		\vpartition[nstr=5,type=2]{{1,-1}}
		\vpartition[type=2]{{3,1,-1},{2,-4},{-2,-3,4},{5,-5}}
		\begin{tikzpicture}
			\vpartition[nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,style=solid,bend=-45]{{1,1},{3,1}}
			\tie[snake=true,style=solid]{{2,1},{4,0}}
			\tie[snake=true,style=solid]{{2,0},{3,0},{4,1}}
			\tie[snake=true,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethione}{
	\ifnum\aspdf=1\[\begin{array}{rrr}
		e\,\,=\vcdraw{\includegraphics{pics/078.pdf}}\qquad\,&
		e'\,\,=\vcdraw{\includegraphics{pics/079.pdf}}\qquad\,&
		r\,\,=\vcdraw{\includegraphics{pics/080.pdf}}\\[1cm]	
		g^*\,\,=\vcdraw{\includegraphics{pics/076-2.pdf}}\qquad\,&
		g^*_p\,\,=\vcdraw{\includegraphics{pics/077-3.pdf}}\qquad\,&
		x_g\,\,=\vcdraw{\includegraphics{pics/077-1.pdf}}
	\end{array}\]\else\[
		\vpartition[type=2]{{1,-3},{-1,3},{4,-4}}
		\vpartition[type=2]{{1,-1},{2,-4},{-2,4},{5,-5}}
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=2]{{1,-1},{2,-2},{3,-3},{4,-4},{5,-5}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{1,3}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=2]{{1,-1},{2,-2},{3,-3},{4,-4},{5,-5}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{2,3}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=2]{{1,-1},{-3,3},{5,-5}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{2,0},{4,1}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{2,1},{4,0}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[tkzpic=0,type=2]{{1,-1},{5,-5}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{2,0},{4,1}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{2,1},{4,0}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{3,1},{3,0}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[,nstr=5,tkzpic=0,type=2]{{1,-1}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{2,0},{2,1}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{4,1},{4,0}}
			\tie[
				snake=true,
				snakelen=4,
				style=solid
			]{{5,1},{5,0}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethitwo}{
	\ifnum\aspdf=1\[	g\,\,\,\,=\,\,
		%\vcdraw{\includegraphics{pics/081-1.pdf}}\,\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/081-5.pdf}}\,\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/081-2.pdf}}\,\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/081-3.pdf}}%\,\,\,\,\,=\,\,\,
		%\vcdraw{\includegraphics{pics/081-4.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\vpartition[floor=3,tkzpic=0,type=1,height=0.7]{{-1,1},{-2,2},{-3,3},{-4,4},{-5,5}}
			\vpartition[floor=2,tkzpic=0,type=0,height=0.7,nstr=5]{{-1,1}}
			\vpartition[floor=1,tkzpic=0,type=0,height=0.7]{{-1,1},{-3,3},{-5,5},{2,-4},{4,-2}}
			\vpartition[tkzpic=0,type=-1,height=0.7]{{-1,1},{-2,2},{-3,3},{-4,4},{-5,5}}
			\tie[
				floor=0,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid
			]{2,3}
			%\tie[
			%	height=0.7,
			%	snake=true,
			%	snakelen=4,
			%	style=solid
			%]{{2,0},{4,1}}
			%\tie[
			%	height=0.7,
			%	snake=true,
			%	snakelen=4,
			%	style=solid
			%]{{4,0},{2,1}}
			\tie[
				floor=2,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid
			]{{2,0},{2,1}}
			\tie[
				floor=2,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid
			]{{4,0},{4,1}}
			\tie[
				floor=2,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid
			]{{5,0},{5,1}}
			\tie[
				floor=3,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid
			]{1,3}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethithr}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/086.pdf}}\,\,\,=\,\,
		\vcdraw{\includegraphics{pics/087.pdf}}\kern+3.5em
		\vcdraw{\includegraphics{pics/088.pdf}}\,\,\,=\,\,
		\vcdraw{\includegraphics{pics/089.pdf}}\,\,\,=\,\,
		\vcdraw{\includegraphics{pics/090.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={},
				customlabelsbelow={b,},
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1}}
			\vpartition[
				customlabelsabove={,a},
				customlabelsbelow={},
				floor=1,
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1,-1}}
			\tie[
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid,
				width=1
			]{{1,0},{2,1}}
			\node at(0.51,1){$\ldots$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={},
				customlabelsbelow={b,},
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{-1,2}}
			\vpartition[
				customlabelsabove={,a},
				customlabelsbelow={},
				floor=1,
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1,-1}}
			\node at(0.51,1){$\ldots$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={},
				customlabelsbelow={b,},
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1}}
			\vpartition[
				customlabelsabove={,a},
				customlabelsbelow={},
				floor=1,
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1,-1}}
			\tie[
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid,
				width=1
			]{{1,0},{2,1}}
			\tie[
				floor=1,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid,
				width=1
			]{{2,0},{2,1}}
			\node at(0.51,1){$\ldots$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={},
				customlabelsbelow={b,},
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{-1,2}}
			\vpartition[
				customlabelsabove={,a},
				customlabelsbelow={},
				floor=1,
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1,-1}}
			\tie[
				floor=1,
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid,
				width=1
			]{{2,0},{2,1}}
			\node at(0.51,1){$\ldots$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[
				customlabelsabove={},
				customlabelsbelow={b,},
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1}}
			\vpartition[
				customlabelsabove={,a},
				customlabelsbelow={},
				floor=1,
				height=0.7,
				nstr=2,
				tkzpic=0,
				type=6,
				width=1
			]{{1,-1},{2,-2}}
			\tie[
				height=0.7,
				snake=true,
				snakelen=4,
				style=solid,
				width=1
			]{{1,0},{2,1}}
			\node at(0.51,1){$\ldots$};
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethifou}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/091.pdf}}
		\,\,\,\,\,=\,\,\,
		\vcdraw{\includegraphics{pics/092.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\strands[
				height=0.6,
				tkzpic=0,
				type=0,
				width=1]{r0*i1*r1}
			\tie[
				height=1.8,
				snake=true,
				snakelen=4,
				style=solid,
				width=1,
			]{1,2}
			\filldraw(0,0.6)circle(0.04);
			\filldraw(1,0.6)circle(0.04);
			\filldraw(0,1.2)circle(0.04);
			\filldraw(1,1.2)circle(0.04);
			\node at(0.5,1.5){$\ldots$};
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[
				height=0.6,
				tkzpic=0,
				type=0,
				width=1]{r0*r0-r1*r1}
			\tie[
				floor=1,
				height=0.6,
				snake=true,
				snakelen=4,
				style=solid,
				width=1,
			]{{1,0},{2,1}}
			\tie[
				floor=1,
				height=0.6,
				snake=true,
				snakelen=4,
				style=solid,
				width=1,
			]{{1,1},{2,0}}
			\node at(0.5,1.5){$\ldots$};
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethifiv}[1]{
	\ifnum\aspdf=1\[
		g\,=\vcdraw{\includegraphics{pics/093.pdf}}\qquad
		g_p\,=\,s\,=\,\vcdraw{\includegraphics{pics/094.pdf}}\qquad
		t\,=\vcdraw{\includegraphics{pics/095.pdf}}\,=\,
		\vcdraw{\includegraphics{pics/096.pdf}}
	\]#1\[g\,\,=\,\vcdraw{\includegraphics{pics/097.pdf}}\]\else\[
		\vpartition[height=1.2,type=2]{{1,-4},{3,-3},{5,-5},{6,-1}}
		\permutation[height=1.2,type=2]{4,2,3,6,5,1}
		\permutation[height=1.2,type=2]{2,3,1}
		\begin{tikzpicture}
			\permutation[bullb=0,floor=1,height=0.6,type=1,tkzpic=0]{1,3,2}
			\permutation[height=0.6,type=-1,tkzpic=0]{2,1,3}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[floor=2,height=0.6,nstr=6,type=1,tkzpic=0]
			{{1,-1},{3,-3},{5,-5},{6,-6}}
			\permutation[bulla=0,bullb=0,floor=1,height=0.6,type=0,tkzpic=0]{1,2,3,6,5,4}
			\permutation[height=0.6,type=-1,tkzpic=0]{4,2,3,1,5,6}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurethisix}{
	\includegraphics{pics/103.pdf}\qquad
	\includegraphics{pics/104.pdf}\qquad
	\includegraphics{pics/105.pdf}\qquad
	\includegraphics{pics/106.pdf}\qquad
	\includegraphics{pics/107.pdf}
}

\newcommand{\figurethisev}{
	\ifnum\aspdf=1
		\[\begin{array}{c}
			\includegraphics{pics/136.pdf}\\[0.3cm]
			\includegraphics{pics/137.pdf}\quad
			\includegraphics{pics/138.pdf}\quad
			\includegraphics{pics/139.pdf}\quad
			\includegraphics{pics/140.pdf}\quad
			\includegraphics{pics/141.pdf}
		\end{array}\]
%		\[\begin{array}{c}
%			\includegraphics[scale=0.9]{pics/130.pdf}\\
%			\includegraphics[scale=0.9]{pics/131.pdf}\quad
%			\includegraphics[scale=0.9]{pics/132.pdf}\quad
%			\includegraphics[scale=0.9]{pics/133.pdf}\quad
%			\includegraphics[scale=0.9]{pics/134.pdf}\quad
%			\includegraphics[scale=0.9]{pics/135.pdf}
%		\end{array}\]
		%\includegraphics{pics/119.pdf}
%		\begin{tikzpicture}
%			\node at(-6,0.1){$_\text{(a)}$};
%			\node at(-6,-2){$_\text{(b)}$};
%			\node at(0,2){\includegraphics{pics/108.pdf}};
%			\node at(-4.6,0){\includegraphics{pics/109.pdf}};
%			\node at(-2.3,0){\includegraphics{pics/110.pdf}};
%			\node at(0,0){\includegraphics{pics/111.pdf}};
%			\node at(2.3,0){\includegraphics{pics/112.pdf}};
%			\node at(4.6,0){\includegraphics{pics/113.pdf}};
%			\node at(-1,-2.2){\includegraphics{pics/114.pdf}};
%			\node at(1,-2.2){\includegraphics{pics/115.pdf}};
%			\draw[line width=0.2,-stealth](-0.1,-0.75)--(-0.70,-1.25);
%			\draw[line width=0.2,-stealth](0.28,-0.75)--(0.84,-1.25);
%		\end{tikzpicture}
	\else
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=4,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
		\end{tikzpicture}
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0},{5,0}}
		\end{tikzpicture}
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{2,0},{5,0}}
		\end{tikzpicture}
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid]{{4,1},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}%[scale=0.9]
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{2,-2}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0}}
%		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=6,type=2,tkzpic=0]{{2,-2}}
%			\tie[color=blue,style=solid]{{6,0},{6,1}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0},{6,0}}
%		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=6,type=2,tkzpic=0]{{2,-2}}
%			\tie[color=blue,style=solid]{{6,0},{6,1}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,0},{6,0}}
%		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=6,type=2,tkzpic=0]{{2,-2}}
%			\tie[color=blue,style=solid]{{6,0},{6,1}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0}}
%			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{4,1},{6,1}}
%		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=6,type=2,tkzpic=0]{{2,-2}}
%			\tie[color=blue,style=solid]{{6,0},{6,1}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0}}
%			\tie[snake=true,snakelen=3,style=solid]{{5,1},{6,1}}
%		\end{tikzpicture}
%		\begin{tikzpicture}[scale=0.9]
%			\vpartition[font=0.5,nstr=6,type=2,tkzpic=0]{{2,-2}}
%			\tie[color=blue,style=solid]{{6,0},{6,1}}
%			\tie[snake=true,snakelen=3,style=solid,bend=45]{{4,1},{2,1}}
%			\tie[snake=true,snakelen=3,style=solid]{{4,0},{5,0}}
%		\end{tikzpicture}
	\fi
}

\newcommand{\figurethieig}{
	\ifnum\aspdf=1\[
		%\vcdraw{\includegraphics{pics/116.pdf}}\quad=\quad
		%\vcdraw{\includegraphics{pics/117.pdf}}\quad=\quad
		%\vcdraw{\includegraphics{pics/118.pdf}}
		\vcdraw{\includegraphics{pics/149.pdf}}\quad=\quad
		\vcdraw{\includegraphics{pics/150.pdf}}\quad=\quad
		\vcdraw{\includegraphics{pics/151.pdf}}
	\]\else
		\begin{tikzpicture}
			\vpartition[height=2,nstr=5,tkzpic=0,type=2]{{1,-1}}
			\tie[height=2,snake=true,snakelen=4,style=solid,bend=-30]{{1,1},{3,1}}
			\tie[height=2,snake=true,snakelen=4,style=solid]{{2,0},{4,1}}
			\tie[height=2,snake=true,snakelen=4,style=solid]{{4,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[floor=3,height=0.5,nstr=5,tkzpic=0,type=1]{{1,-1},{4,-4},{5,-5}}
			\vpartition[bulla=0,height=1.5,nstr=5,tkzpic=0,type=-1]{{1,-1}}
			\tie[floor=3,height=0.5,snake=true,snakelen=4,style=solid,bend=-30]{{1,1},{3,1}}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{2,1},{3,0}}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{2,0},{4,1}}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{3,1},{5,0}}
			\tie[height=1.5,snake=true,snakelen=4,style=solid]{{4,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[floor=3,height=0.5,nstr=5,tkzpic=0,type=1]{{1,-1},{3,-3},{4,-4},{5,-5}}
			\vpartition[floor=2,bulla=0,height=0.5,nstr=5,tkzpic=0,type=0]{{1,-1},{4,-4},{5,-5}}
			\vpartition[floor=1,bulla=0,height=0.5,nstr=5,tkzpic=0,type=0]{{1,-1},{2,-2},{5,-5}}
			\vpartition[bulla=0,height=0.5,nstr=5,tkzpic=0,type=-1]{{1,-1},{2,-2},{4,-4}}
			\tie[floor=2,height=0.5,snake=true,snakelen=4,style=solid]{{1,1.5},{2,1.5},{3,1.5}}
			\tie[height=0.5,snake=true,snakelen=4,style=solid]{{2,2},{3,2},{4,2}}
			\tie[height=0.5,snake=true,snakelen=4,style=solid]{{4,1},{5,1}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figurethinin}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/120.pdf}}\qquad
		\vcdraw{\includegraphics{pics/121.pdf}}\qquad
		\vcdraw{\includegraphics{pics/122.pdf}}
	\]\else
		\begin{tikzpicture}
			\vpartition[floor=2,height=0.5,nstr=4,tkzpic=0,type=1]{{4,-4}}
			\vpartition[bulla=0,bullb=0,floor=1,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1},{2,-2},{3,-3},{4,-4}}
			\vpartition[height=0.5,nstr=4,tkzpic=0,type=-1]{{1,-1}}
			\tie[floor=1,height=0.5,snake=true,snakelen=4,style=solid]{1,2,3,4}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[floor=2,height=0.5,nstr=4,tkzpic=0,type=1]{{1,-1}}
			\vpartition[bulla=0,bullb=0,floor=1,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1},{2,-2},{3,-3},{4,-4}}
			\vpartition[height=0.5,nstr=4,tkzpic=0,type=-1]{{4,-4}}
			\tie[floor=1,height=0.5,snake=true,snakelen=4,style=solid]{1,2,3,4}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[floor=2,height=0.5,nstr=4,tkzpic=0,type=1]{{1,-1},{4,-4}}
			\vpartition[bulla=0,bullb=0,floor=1,height=0.5,nstr=4,tkzpic=0,type=0]{{1,-1},{2,-2},{3,-3},{4,-4}}
			\vpartition[height=0.5,nstr=4,tkzpic=0,type=-1]{{1,-1},{4,-4}}
			\tie[floor=1,height=0.5,snake=true,snakelen=4,style=solid]{1,2,3,4}
		\end{tikzpicture}
	\fi
}

\newcommand{\figureforty}{
	\ifnum\aspdf=1\[\begin{array}{c}
		\vcdraw{\includegraphics{pics/124.pdf}}\qquad
		\vcdraw{\includegraphics{pics/125.pdf}}\qquad
		\vcdraw{\includegraphics{pics/126.pdf}}\\[0.9cm]
		\vcdraw{\includegraphics{pics/127.pdf}}\qquad
		\vcdraw{\includegraphics{pics/128.pdf}}\qquad
		\vcdraw{\includegraphics{pics/129.pdf}}
	\end{array}\]\else
		\vpartition[height=1,type=2]{{1,2},{3,-1},{-2,-4}}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2},{3,-1},{-2,-4}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2,5},{3,-1},{-2,-4}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2},{5,3,-1},{-2,-4}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2},{3,-1},{4,5},{-2,-4}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2},{3,-1},{-2,-4,-5}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[height=1,tkzpic=2,type=2,nstr=5]{{1,2},{3,-1},{-2,-4},{-3,-5}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figureforone}{
	\ifnum\aspdf=1
		\[\begin{array}{c}
			\includegraphics{pics/142.pdf}\\[0.3cm]
			\includegraphics{pics/143.pdf}\quad
			\includegraphics{pics/144.pdf}\quad
			\includegraphics{pics/145.pdf}\quad
			\includegraphics{pics/146.pdf}\quad
			\includegraphics{pics/147.pdf}
		\end{array}\]
	\else
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[color=blue,style=solid]{{5,0},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1},{5,-5}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
			\tie[snake=true,snakelen=3,style=solid]{{5,0},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{5,0},{2,0}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0},{5,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vpartition[font=0.5,nstr=5,type=2,tkzpic=0]{{1,-1}}
			\tie[snake=true,snakelen=3,style=solid,bend=45]{{3,1},{1,1}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid,bend=-45]{{3,1},{5,1}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figurefortwo}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/154.pdf}}
		\quad\,\,=\quad
		\vcdraw{\includegraphics{pics/155.pdf}}
	\]\else
		\begin{tikzpicture}
			\arcpartition[bend=55,num=9,tkzpic=0,type=0]{{1,2,8},{4,7},{5,6}}
			\arcpartition[bend=-55,bull=0,tkzpic=0,type=0]{{1,4},{5,9},{6,8}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\arcpartition[bend=55,num=9,tkzpic=0,type=0]{{1,2,8},{4,7},{5,6}}
			\arcpartition[bend=-55,bull=0,tkzpic=0,type=0]{{1,5},{6,9},{7,8}}
		\end{tikzpicture}
	\fi
}

\newcommand{\figureforthr}{
	\ifnum\aspdf=1\[\left(
		\vcdraw{\includegraphics{pics/156.pdf}}\,\,\,,
		\vcdraw{\includegraphics{pics/157.pdf}}\,\right)\quad=\quad
		\vcdraw{\includegraphics{pics/158.pdf}}
	\]\else\[
		\vcdraw{\begin{tikzpicture}
			\arcpartition[norma=0.9,bend=70,tkzpic=0,type=1]{{1,6},{2,5},{3,4}}
		\end{tikzpicture}}
		\vcdraw{\begin{tikzpicture}
			\arcpartition[norma=0.9,bend=70,tkzpic=0,type=1]{{1,2,3,4,5,6}}
		\end{tikzpicture}}
		\vcdraw{\begin{tikzpicture}
			\arcpartition[norma=0.9,bend=70,tkzpic=0,type=1]{{1,6},{2,5},{3,4}}
			\tie[snake=true,snakelen=3,style=solid]{{3.5,0.165},{3.5,0.49},{3.5,0.82}}
		\end{tikzpicture}}
		\]
	\fi
}

\newcommand{\figureforfor}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/159.pdf}}\kern+0.7em\to\kern+0.1em
		\vcdraw{\includegraphics{pics/160.pdf}}\quad\!\to\!\quad
		\vcdraw{\includegraphics{pics/161.pdf}}
	\]\else\[
		\vcdraw{\begin{tikzpicture}
			\path[rounded corners,draw=white,fill=gray!30]
				(5.65,0)to[bend right=75]
				(-0.25,0)to
				(-0.25,-0.5)to
				(2.5,-0.5)to			
				(2.7,0.15)to
				(2.9,-0.5)to
				(5.65,-0.5)--cycle;
			\arcpartition[
				customlabels={1,2,3,4,5,5,4,3,2,1},
				bend=70,
				norma=3.3,
				tkzpic=0,
				type=-6
			]{{1,8},{9,10},{2,3},{4,7},{5,6}}
			\tie[snake=true,snakelen=3,style=solid]{{5.5,0.49},{5.5,1.09}}
			\tie[snake=true,snakelen=3,style=solid]{{2.5,0.17},{2.5,0.9}}
			\tie[bend=-50,snake=true,snakelen=3,style=solid]{{9.5,0.17},{7.5,0.49}}
		\end{tikzpicture}}
		\vcdraw{\begin{tikzpicture}
			\path[rounded corners,draw=white,fill=gray!30]
				(3.45,3.3)to[bend right=50]
				(-0.25,-0.5)to
				(2.68,-0.5)to[bend left=50]
				(3.45,0.27)--cycle;
			\arcpartition[
				customlabels={1,2,3,4,5},
				bend=70,
				norma=3.3,
				num=5,
				tkzpic=0,
				type=-6
			]{{2,3}}
			\filldraw(3,0.6)circle(0.04);\node[scale=0.5]at(3.2,0.6){5};
			\filldraw(3,1.2)circle(0.04);\node[scale=0.5]at(3.2,1.2){4};
			\filldraw(3,1.8)circle(0.04);\node[scale=0.5]at(3.2,1.8){3};
			\filldraw(3,2.4)circle(0.04);\node[scale=0.5]at(3.2,2.4){2};
			\filldraw(3,3.0)circle(0.04);\node[scale=0.5]at(3.2,3.0){1};
			\draw[bend right=-70,line width=0.7](3,2.4)to(3,3.0);	
			\draw[bend right=-50,line width=0.7](2.4,0)to(3,0.6);	
			\draw[bend right=-50,line width=0.7](1.8,0)to(3,1.2);	
			\draw[bend right=-50,line width=0.7](0.0,0)to(3,1.8);	
			\tie[snake=true,snakelen=3,style=solid]{{2.5,0.17},{2.5,1.45}}
			\tie[bend=40,snake=true,snakelen=3,style=solid]{{4.5,0.85},{4,1.86}}
			\tie[bend=-40,snake=true,snakelen=3,style=solid]{{5.72,2.69},{5,1.91}}
		\end{tikzpicture}}
		\vcdraw{\begin{tikzpicture}
			\path[rounded corners,draw=white,fill=gray!30]
				(-0.25,3.3)to
				(-0.25,-0.5)to
				(2.68,-0.5)to
				(2.68,3.3)--cycle;
			\vvpartition[bend=70,height=2.8,norma=3.3,type=2]{{1,2},{3,-1},{-2,-3},{4,-4},{5,-5}}
			\tie[bend=-40,snake=true,snakelen=3,style=solid]{{1.5,2.63},{2.64,2.3}}
			\tie[bend=-40,snake=true,snakelen=3,style=solid]{{2.5,0.17},{1.36,0.5}}
			\tie[snake=true,snakelen=3,style=solid]{{2,1.4},{4,1.4}}
		\end{tikzpicture}}
		\]
	\fi
}

\newcommand{\figureforfiv}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/043.pdf}}\!\!\cdots\!\!
		\vcdraw{\includegraphics{pics/162.pdf}}\cdots\!\!
		\vcdraw{\includegraphics{pics/043.pdf}}\]
	\else\[
		\begin{tikzpicture}
			\strands[nstr=4,type=0,tkzpic=0]{t2}
			\tie[snake=true,snakelen=3,style=solid]{{2.5,0.295},{2.5,0.705}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figureforsix}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/163.pdf}
	\]\else\[
		\vpartition[
			height=1.5,
			type=6,
			customlabelsabove={,2,3,,,,7,8},
			customlabelsbelow={16,15,14,,12,,,}]
		{{1,2},{3,-1},{4,-8},{5,8},{6,7},{-2,-7},{-3,-4},{-5,-6}}
	\]\fi
}

\newcommand{\figureforsev}{
	\ifnum\aspdf=1\[
		\includegraphics{pics/164.pdf}\kern+4em
		\includegraphics{pics/165.pdf}
	\]\else\[
		\begin{tikzpicture}
			\vvpartition[height=1.3,type=2]{{1,2},{3,-1},{4,5},{6,-8},{7,8},{-2,-3},{-4,-7},{-5,-6}}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,1.175},{1.5,0.33}}
			\tie[snake=true,snakelen=3,style=solid]{{2.5,0.125},{2.5,0.975}}
			\tie[snake=true,snakelen=3,style=solid]{{4.5,1.175},{4.5,0.23}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vvpartition[height=1.3,type=2]{{1,2},{3,-1},{4,5},{6,-8},{7,8},{-2,-3},{-4,-7},{-5,-6}}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,1.175},{1.5,0.33}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[snake=true,snakelen=3,style=solid]{{2,0.65},{7,0.65}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figureforeig}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/166.pdf}}\quad=\quad
		\vcdraw{\includegraphics{pics/167.pdf}}
	\]\else\[
		\vpartition[bend=70,height=3.6,type=2]{{1,2},{3,-1},{4,-8},{5,8},{6,7},{-2,-7},{-3,-4},{-5,-6}}
		\strands[height=0.9,type=2]{t1-t6*t5-t7*t2-t4-t6*t3-t5}
	\]\fi
}

\newcommand{\figurefornin}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/168.pdf}}\quad=\quad
		\vcdraw{\includegraphics{pics/169.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\vvpartition[bend=70,height=2.7,type=2]{{1,2},{3,-1},{4,5},{6,-8},{7,8},{-2,-3},{-4,-7},{-5,-6}}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,2.535},{1.5,0.68}}
			\tie[snake=true,snakelen=3,style=solid]{{2.5,0.158},{2.5,2.04}}
			\tie[snake=true,snakelen=3,style=solid]{{4.5,2.535},{4.5,0.34}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=0.9,tkzpic=0,type=2]{t1-t7*t2-t4-t6*t5}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,2.43},{1.5,2.07}}
			\tie[snake=true,snakelen=3,style=solid]{{2.5,1.53},{2.5,1.17}}
			\tie[snake=true,snakelen=3,style=solid]{{4.5,1.53},{4.5,1.17}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurefifty}{
	\ifnum\aspdf=1\[
		\begin{array}{cccc}		
			&\vcdraw{\includegraphics{pics/170.pdf}}
			&\to
			&\vcdraw{\includegraphics{pics/171.pdf}}\\[1.5cm]
			\to
			&\vcdraw{\includegraphics{pics/172.pdf}}
			&\to
			&\vcdraw{\includegraphics{pics/173.pdf}}
		\end{array}
	\]\else\[
		\begin{tikzpicture}
			\vvpartition[bend=45,height=1.5,type=2]{{1,2},{3,-1},{4,5},{6,-8},{7,8},{-2,-3},{-4,-7},{-5,-6}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{1.5,0.916},{1.5,0.25}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{3,0},{4,0}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{2.3,0.65},{6.7,0.65}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\vvpartition[bend=45,height=1.5,type=2]{{1,2},{3,6},{4,5},{7,8},{-1,-8},{-2,-7},{-3,-4},{-5,-6}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{1.5,0.916},{1.5,0.17}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{3.5,0.08},{3.5,0.353}}
			\tie[height=1.5,snake=true,snakelen=3,style=solid]{{4.5,0.578},{4.5,0.75}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=0.9,tkzpic=0,type=2]{t1-t4*t3-t5-t7*t2-t4-t6*t3-t5}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,2.97},{1.5,3.33}}
			\tie[snake=true,snakelen=3,style=solid]{{3.5,0.27},{3.5,0.63}}
			\tie[snake=true,snakelen=3,style=solid]{{3.5,2.07},{3.5,2.43}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=0.9,tkzpic=0,type=2]{t1-t4*t5-t7*t2-t4-t6*t5}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,2.97},{1.5,3.33}}
			\tie[snake=true,snakelen=3,style=solid]{{3,0.45},{4,0.45}}
			\tie[snake=true,snakelen=3,style=solid]{{3,2.25},{4,2.25}}
		\end{tikzpicture}
	\]\fi
}

\newcommand{\figurefifone}{
	\ifnum\aspdf=1\[
		\vcdraw{\includegraphics{pics/174.pdf}}\to
		\vcdraw{\includegraphics{pics/175.pdf}}\to
		\vcdraw{\includegraphics{pics/176.pdf}}\to
		\vcdraw{\includegraphics{pics/177.pdf}}
	\]\else\[
		\begin{tikzpicture}
			\strands[height=2.55,nstr=6,tkzpic=0,type=2]{t2-t4}
			\tie[height=2.55,snake=true,snakelen=3,style=solid]{1,6}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=2.55,nstr=6,tkzpic=0,type=2]{r0-t2-t4-r5}
			\tie[color=black,height=2.55,style=solid,bend=-65,tiewidth=0.7]{{1,1},{6,1}}
			\tie[color=black,height=2.55,style=solid,bend=+65,tiewidth=0.7]{{1,0},{6,0}}
			\tie[height=2.55,snake=true,snakelen=3,style=solid]{{3.5,0.31},{3.5,0.69}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=0.85,tkzpic=0,type=2]{t2-t4*t1-t3-t5*t2-t4}
			\tie[snake=true,snakelen=3,style=solid]{{1.5,1.135},{1.5,1.415}}
		\end{tikzpicture}
		\begin{tikzpicture}
			\strands[height=0.85,tkzpic=0,type=2]{t2-t4*t3-t5*t2-t4}
			\tie[height=2.55,snake=true,snakelen=3,style=solid]{{1,0.5},{2,0.5}}
		\end{tikzpicture}
	\]\fi
}

